CRAFT: ClusteR-specific Assorted Feature selecTion

We present a framework for clustering with cluster-specific feature selection. The framework, CRAFT, is derived from asymptotic log posterior formulations of nonparametric MAP-based clustering models. CRAFT handles assorted data, i.e., both numeric and categorical data, and the underlying objective functions are intuitively appealing. The resulting algorithm is simple to implement and scales nicely, requires minimal parameter tuning, obviates the need to specify the number of clusters a priori, and compares favorably with other methods on real datasets.

==> abstract_V.tex <==

\begin{abstract} 
We present an unsupervised framework for clustering with cluster-specific feature selection. The framework, CRAFT, is derived from asymptotic log posterior formulations of nonparametric MAP-based clustering models. CRAFT handles assorted data, i.e., both numeric and categorical data, and the underlying objective functions are intuitively appealing. The resulting algorithm is very simple to implement and scales nicely, requires minimal parameter tuning, and obviates the need to specify the number of clusters a priori. Besides, CRAFT outperforms the state-of-the-art unsupervised methods on several real world benchmark datasets.      
\end{abstract} 

%---------- This was the ICML abstract

%We present a framework for clustering with cluster-specific feature selection. The framework is derived from asymptotic log posterior formulations of nonparametric MAP-based clustering models. Besides handling assorted data, i.e. both numeric and categorical data, the proposed method (a) can be viewed as a subspace clustering method since it allows for cluster-specific feature selection, (b) provides adjustable parameters that extract a desired number of features in the subspaces, and enable global or local feature selection as required, and (c) obviates the need to specify the number of clusters a priori. Additionally, the underlying objective functions are intuitively appealing, and the resulting algorithms are very simple to implement and scale nicely like the K-means algorithm. We also provide comprehensive experimental evidence to demonstrate the efficacy of the proposed framework. 

%-----------------------------------





 %Feature or variable selection continues to take center stage in machine learning owing to its fundamental benefits such as enhanced model interpretability, reduced data storage and processing effort, and improved generalization for predictions. 

==> description_V2.tex <==
\section{The CRAFT Framework}\label{SectionCRAFTWithFS}
Recently, \citet{Broderick} derived several variants of the nonparametric $K$-means objective under asymptotic conditions, i.e., when the underlying Gaussian distributions converge to a deterministic point distribution. We significantly build on  this work to develop a principled methodology to achieve cluster-specific feature selection on heterogeneous data. The main intuition behind our formalism is that the points in a cluster should agree closely on the selected features, which it turns out, is closely related to their entropy for discrete data and variance for numeric data. For instance, consider a nonparametric setting where the features are all binary categorical, i.e. they take values only in the set $\{0, 1\}$, and we select all the features. Assume that the features are drawn from independent Bernoulli distributions. Then assuming the number of clusters is $K^+$, where $K^+$ depends on the cluster assignment vector $z$,  we obtain the following objective using a straightforward maximum likelihood estimation (MLE) procedure:    % and  
\small \begin{eqnarray*}\label{BinaryClusterObjective2}
\arg\!\min_{z}\,\,  \sum_{k=1}^{K^+(z)} \sum_{n: z_{n, k} = 1}  \sum_{d} \mathbb{H}(\mu_{kd}^*)  +  \lambda K^+(z),  
\end{eqnarray*} \normalsize
where $\mu_{kd}^*$ denotes the mean of feature $d$ computed by using points belonging to cluster $k$, and the entropy function $\mathbb{H}(p)  =  -p \log p - (1 - p) \log (1 - p)\, \text{ for } p \in [0, 1]$ characterizes the uncertainty. For a fixed number of clusters, the objective tries to minimize the overall uncertainty across clusters and thus forces similar points to come together, which makes sense from a clustering perspective.  

However, it is not immediately clear how we can extend this insight about clustering to cluster-specific feature selection. A main technical novelty of our work is to combine assorted data by enforcing a common Bernoulli prior on the selected features, and derive an asymptotic approximation for the posterior joint log likelihood of the observed data, cluster indicators, cluster means, and feature means.  Additional modeling assumptions can be made for individual data types independent of the other types. Essentially, the asymptotics then allow us to ``interpolate" between the MLE and maximum a priori (MAP) estimates. Unlike Variational Bayes methods, that are typically computationally intensive, our formulation leads to an elegant K-means style algorithm that has following steps repeated: (a) compute the ``distances"  to the cluster centers using the selected features for each cluster, choose which cluster each point should be assigned (and create new clusters if needed), and recompute the centers and select the appropriate cluster-specific features for the next iteration. 

We set up the problem as follows. The data $x$ consists of $N$ i.i.d. D-dimensional binary vectors $x_1, x_2, \ldots, x_N$.  We assume a Dirichlet process (DP) mixture model  to avoid having to specify apriori the number of clusters $K^{+}$, and use the hyper-parameter $\theta$, in the underlying exchangeable probability partition function (EFPF) \cite{Pitman}, to tune the probability of starting a new cluster.   We use $z$ to denote cluster indicators:  $z_{n, k} = 1$ if $x_n$ is assigned to cluster $k$, and $\mathbb{H}(\cdot)$ to denote the entropy function. Since $K^+$ depends on $z$, we will often make the connection explicit by writing $K^+(z)$. Let $Cat$ and $Num$ denote respectively the set of categorical and the set of numeric features respectively.

For categorical features, we assume the features $d$ selected in any cluster $k$ are drawn from a discrete distribution with parameters $\eta_{kdt},\, d \in Cat$, where $t \in \mathcal{T}_{d}$ indexes the different values taken by the categorical feature $d$. In turn, we assume the parameters $\eta_{kdt}$ are drawn from a Beta distribution with parameters $\alpha_{kdt}/K^+$ and 1. On the other hand, we assume the features not selected to have been drawn from a discrete distribution with cluster-independent parameters $\eta_{0dt}$. The variables $v_{kd} \in \{0, 1\}$ indicate whether feature $d \in [D]$ is selected in cluster $k \in [K]$. We assume $v_{kd}$ is generated from a Bernoulli distribution with parameter $\nu_{kd}$. Further, we assume $\nu_{kd}$ is generated from a Beta prior having variance $\rho$ and mean $m$, as shown in Fig. \ref{fig:FDPCRAFT_mix-Graphical}. We assume features $d$ that have not been selected are drawn from a discrete distribution with cluster-independent mean $\eta_{0dt}$.%, i.e., the average value of the feature over all points in the dataset. 

For numeric features, we formalize the intuition that the features selected to represent clusters should exhibit small variance asymptotics relative to global, by assuming a conditional density of the form:
$$f(x_{nd}|v_{kd}) = \dfrac{1}{Z_{kd}} e^{-\left[v_{kd}(x_{nd}-\zeta_{kd})^2 + (1-v_{kd}) \sigma_{kd}^2(x_{nd}-\zeta_{d})^2\right]}, \,\,\,\,  Z_{kd} = \dfrac{\sqrt{\pi}(\sigma_{kd}+1)}{\sigma_{kd}},$$
where $x_{nd} \in \mathbb{R}$, $v_{kd} \in \{0, 1\}$, and $Z_{kd}$ ensures $f$ integrates to 1, and $\sigma_{kd}$ guides the allowed variance of a selected feature $d$ over points in cluster $k$ by asserting feature $d$ concentrate around its cluster mean $\zeta_{kd}$. The features not selected are assumed to be drawn from Gaussian distributions that have variances $1/\sigma_{kd}^2$ and cluster independent means $\zeta_d$. Fig. \ref{fig:FDPCRAFT_mix-Graphical} shows the resulting graphical model.   Let $\mathbb{I}(\mathcal{P})$ be 1 if the predicate $\mathcal{P}$ is true, and 0 otherwise. Under asymptotic conditions, minimizing the joint negative log-likelihood yields the following objective (see the Supplementary for details):  

\small
\begin{eqnarray}\nonumber \label{Discrepancy} 
\arg\!\!\!\min_{z, v, \eta, \zeta}\, \underbrace{\sum_{k=1}^{K^+} \sum_{n: z_{n, k} = 1}  \sum_{d \in Num} v_{kd} (x_{nd} - \zeta_{kd})^2}_{\text{Numeric Data Discrepancy}} + \underbrace{(\lambda + DF_0) K^+}_{\text{Regularization Term}} + \underbrace{\left(\displaystyle \sum_{k=1}^{K^+} \sum_{d= 1}^{D} v_{kd}\right) F_{\Delta}}_{\text{Feature Control}}, \\
+ \underbrace{\sum_{k=1}^{K^+} \sum_{d \in Cat} \left[v_{kd} \left(\sum_{n: z_{n, k} = 1} - \mathbb{I}(x_{nd} = t) \log \eta_{kdt})\right) + (1-v_{kd}) \sum_{n: z_{n, k} = 1} \sum_{t \in \mathcal{T}_d}  - \mathbb{I}(x_{nd} = t) \log \eta_{0dt} \right]}_{\text{Categorical Data Discrepancy}} \nonumber 
\end{eqnarray}    \normalsize
where
$F_{\Delta}$ and $F_0$ depend only on the ($m$, $\rho$) pair: $F_{\Delta}  =  F_1 - F_0$, with
\begin{eqnarray} \label{ComputeF}
F_0 & = & (a_0+b_0) \log\, (a_0+b_0) - a_0 \log \, a_0 - b_0 \log \, b_0,   \nonumber\\
F_1 & = & (a_1+b_1) \log\, (a_1+b_1) - a_1  \log \, a_1 - b_1 \log \, b_1, \\
a_0 & = &  \dfrac{m^2(1-m)}{\rho} - m, b_0  =  \dfrac{m(1-m)^2}{\rho} + m, a_{1}   =  a_0 +  1,  \text{ and }\,\,b_1  =  b_0  -  1. \nonumber
\end{eqnarray}


This objective has an elegant interpretation. Besides the discrepancy for categorical data and numeric data, we also have regularization terms to (a) control the number of clusters, and (b) modulate the effect of feature selection.  The feature control term encapsulates the adjustable parameters: $m$ controls the number of features that would be turned on per cluster, whereas $\rho$ guides the extent of cluster-specific feature selection. A detailed derivation is provided in the Supplementary.  


\begin{algorithm}[t]
\caption{CRAFT}          % give the algorithm a caption
\label{alg3}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                    % enter the algorithmic environment
    \REQUIRE $x_1, \ldots, x_N$: $D$-dimensional input data on categorical features $Cat$ and numeric features $Num$,  $\lambda > 0$: regularization parameter,  and $m \in (0, 1)$: fraction of features per cluster, and (optional) $\rho \in (0, m(1-m))$: control parameter that guides global/local feature selection. Each feature $d \in Cat$ takes values from the set $\mathcal{T}_d$, while each feature $d \in Num$ takes values from $\mathbb{R}$.  
    \ENSURE $K^{+}$: number of clusters, $l_1, \ldots, l_{K^+}$: clustering, and $v_1, \ldots, v_{K^+}$: selected features.
    \begin{enumerate} 
     \STATE Initialize $K^+ = 1$, $l_1 = \{x_1, \ldots, x_N\}$, cluster center (sample randomly) with categorical mean $\eta_1$ and numeric mean $\zeta_1$, and draw $v_1 \sim \left[Bernoulli\left(m \right)\right]^D$.  If $\rho$ is not specified as an input, initialize $\rho = \max\{0.01, m(1-m) - 0.01\}$.  Compute the global categorical mean $\eta_{0}$. 
      Initialize the cluster indicators $z_n = 1$ for all $n \in [N]$.
      \STATE Compute $F_{\Delta}$ and $F_0$ using \eqref{ComputeF}.
     \STATE Repeat until cluster assignments do not change
     \begin{itemize}
             \item For each point $x_n$ 
            \begin{itemize}
                \item \hspace*{-0.2 cm} Compute $\forall k \in [K^+]$
              \small  \[\hspace*{-1cm}  d_{nk} = \sum_{d \in Num} v_{kd} (x_{nd} - \zeta_{kd})^2 +  \sum_{d \in Cat: v_{kd} = 0} \sum_{t \in \mathcal{T}_d} - \mathbb{I}(x_{nd} = t) \log \eta_{0dt}  \]\\ \[\hspace*{-0.5cm} +  \displaystyle \left(\sum_{d=1}^Dv_{kd}\right)F_{\Delta}  \,\,+ \displaystyle \sum_{d \in Cat: v_{kd} = 1} \sum_{t \in \mathcal{T}_d} - \mathbb{I}(x_{nd} = t) \log \eta_{kdt}.\] \normalsize
                 \STATE If $\displaystyle \min_k d_{nk} > (\lambda + DF_0)$, set $K^+ = K^+ + 1$, $z_n = K^+$, and draw $$v_{K^+d} \small \sim Bernoulli\left(\dfrac{\sum_{j=1}^{K^+-1} a_{v_{jd}}}{\sum_{j=1}^{K^+-1} (a_{v_{jd}} + b_{v_{jd}})}\right)\,\,\, \forall  d \in [D],$$\normalsize where $a$ and $b$ are as defined in \eqref{ComputeF}. Set $\eta_{K^+}$ and $\zeta_{K^+}$ using $x_n$. 
                 \STATE Otherwise, set $z_n = \displaystyle \arg\!\min_k d_{nk}$. 
            \end{itemize}  
            \item Generate clusters $l_1, \ldots, l_{K^+}$ based on $z_1, \ldots, z_{K^+}$: $l_k = \{x_n \,|\, z_n = k\}$.
            \item Update the means $\eta$ and $\zeta$ for all the clusters.
            \item For each cluster $l_k$, $k \in [K^+]$,  update $v_k$: choose the $m|Num|$ numeric features $d'$  with lowest $\sigma_{kd'}$ in $l_k$, and choose $m|Cat|$ categorical features $d$ with maximum value of $G_{d} - G_{kd}$, where $G_{d} =-\, \sum_{n} \sum_{t \in \mathcal{T}_d} \mathbb{I}(x_{nd} = t) \log \eta_{0dt}$ and $G_{kd} = -\,\sum_{n: z_{n, k} = 1} \sum_{t \in \mathcal{T}_d} \mathbb{I}(x_{nd} = t) \log \eta_{kdt}$. \\
               \end{itemize}
    \end{enumerate}
\end{algorithmic}
\end{algorithm}


\begin{figure*}[t!]
\centering
\input{model_FCAKE_mix}
 \caption{CRAFT- Graphical model. For cluster-specific feature selection $\rho$ is set to a high value determined by $m$, whereas for global feature selection $\rho$ is set close to 0. The dashed arrow emphasizes this significant artifact of our formalism that unifies cluster-specific and global feature selection. \label{fig:FDPCRAFT_mix-Graphical}}
\end{figure*}

A K-means style alternating minimization procedure for clustering assorted data, along with feature selection is outlined in Algorithm \ref{alg3}. The algorithm repeats the following steps until convergence: (a) compute the ``distances" to the cluster centers using the selected features for each cluster, (b) choose which cluster each point should be assigned (and create new clusters if needed), and (c) recompute the cluster centers and select the appropriate features for each cluster using the criteria that follow directly from the model objective and variance asymptotics.  
In particular, the algorithm starts a new cluster if the cost of assigning a point to its closest cluster center exceeds $(\lambda + DF_0)$, the cost it would incur to initialize an additional cluster.  The information available from the already selected features is leveraged to guide the initial selection of features in the new cluster. Finally, the updates on cluster means and feature selection are performed at the end of each iteration.        
 
 \subsubsection*{Approximate Budget Setting for a Variable Number of Features}
Algorithm \ref{alg3} selects an exact fraction of features per cluster, which can be viewed as a fixed budget constraint. However, the CRAFT framework is not limited to this design choice, and Algorithm \ref{alg3} can be modified slightly to allow a variable number of features across clusters. For categorical features, note that selecting the $m$ features having the maximum difference $G_d - G_{kd}$ implicitly imposes a threshold, below which we do not select any features.  Therefore, to accommodate variable number of features, we can transform the multiplicative ratio constraint of  Algorithm \ref{alg3} to an additive one: specify a tuning parameter $\epsilon_c \in (0, 1)$ and choose all the features $d$ in cluster $k$ for which $G_{d} - G_{kd} > \epsilon_c G_{d}$. Likewise for numeric features, we may simply choose features that have variance less than some positive constant $\epsilon_v$.   As we show later, this slightly modified algorithm recovers the exact subspace on synthetic data in the approximate budget setting for a wide range of $m$. Henceforth, we will focus mainly on the fixed budget setting using the outline in Algorithm \ref{alg3}.  %
 
\section{Discussion}
Thus far we focused entirely on the algorithmic aspects of CRAFT.  We now  describe some conceptual underpinnings of CRAFT and their ramifications for the related prior work and future directions. 

\subsubsection*{Recovering DP-means objective on Numeric Data}
When all the features are retained, CRAFT recovers the DP-means objective \cite{Kulis} on numeric data:
\small \begin{eqnarray} \arg\!\min_{z}\,\, \sum_{k=1}^{K^+(z)} \sum_{n: z_{n, k} = 1}  \sum_{d} (x_{nd} - \zeta_{kd}^*)^2 +  \lambda K^+(z), \end{eqnarray} \normalsize 
where $\zeta_{kd}^*$ denotes the (numeric) mean of feature $d$ computed by using points belonging to cluster $k$.
 
\subsubsection*{Unifying Global and Local Feature Selection}
An important aspect of CRAFT is that the point estimate of $\nu_{kd}$ is
$$\dfrac{a_{kd}}{a_{kd}+b_{kd}} = \dfrac{\left(\dfrac{m^2(1-m)}{\rho} - m\right) +  v_{kd}}{\dfrac{m(1-m)}{\rho} } = m + \dfrac{(v_{kd} - m)\rho}{m(1-m)} \to \begin{cases}  v_{kd}, \qquad \mbox{ as } \rho \to m(1 - m)\\ m, \qquad \,\,\, \mbox{ as } \rho \to 0.  \end{cases}$$ 
Thus, using a single parameter $\rho$, we can interpolate between cluster specific selection, $\rho \to m(1 - m)$,  and global selection, $\rho \to 0$. Since we are often interested only in one of these two extreme cases, this also implies that we essentially need to specify only $m$, which is often determined by application requirements. Thus, CRAFT requires minimal tuning for most practical purposes.    

\subsubsection*{Accommodating Statistical-Computational Trade-offs} 
We can easily extend the basic CRAFT model, shown in Fig. \ref{fig:FDPCRAFT_mix-Graphical}  by instead having cluster specific means $m_k$, which may in turn be modulated via Beta priors. The model can also be readily extended to incorporate more informative priors or allow overlapping clusters, e.g., we can do away with the independent distribution assumptions for numeric data, by introducing covariances and taking a suitable prior like the inverse Wishart. The parameters $\alpha$ and $\sigma$ do not appear in the CRAFT objective since they vanish due to the asymptotics and the appropriate setting of the hyperparameter $\theta$. Retaining some of these parameters, in the absence of asymptotics, will lead to additional terms in the objective thereby requiring more computational effort. Depending on the available computational resource, one might also like to achieve feature selection with the exact posterior instead of a point estimate. CRAFT can gracefully accommodate all such statistical-computational trade-offs. 





==> experiments_V2.tex <==
\section{Experimental Results}\label{SectionExperiments}
We conducted extensive experiments on several synthetic and real datasets to validate the CRAFT framework. We first provide empirical evidence on synthetic dat about CRAFT's ability to recover the feature subspaces. We then show how CRAFT outperforms DP-means, which we enhance to include feature selection, on a real binary dataset to underscore the significance of having a different measure for categorical data from numeric data. Finally, we compare CRAFT with other recently proposed feature selection methods on several real world benchmarks to substantiate our framework. We set $\rho = m(1-m) - 0.01$ in all our experiments to facilitate cluster specific feature selection. 


\subsubsection*{Exact Subspace Recovery on Synthetic Data}
We now show the results of our experiments on synthetic data, in  both the fixed and the approximate budget settings,  that suggest CRAFT has the ability to recover subspaces on both categorical and numeric data, amidst noise, under different scenarios:  (a) disjoint subspaces, (b) overlapping subspaces including the extreme case of containment of a subspace wholly within the other, (c) extraneous features,  and (d) non-uniform distribution of examples and features across clusters.  \\ \\
%To verify the efficiency of CRAFT in recovering the features and clusters for both categorical and numeric data, we  generated two synthetic datasets comprising . To facilitate visualization, we used `imagesc' command in MATLAB to color each partition in the original and the recovered matrices.  
\noindent \textbf{Fixed Budget Setting:}
Fig. \ref{subspace1a} shows the first categorical synthetic dataset comprising 300 24-feature points, evenly split between 3 clusters that have disjoint subspaces of 8 features each. We sampled the remaining features independently from a Bernoulli distribution with parameter 0.1. Fig. \ref{subspace1b} shows that CRAFT recovered the subspaces with $m = 0.33$. 
 In Fig. \ref{subspace1c} we modified the dataset to have (a) an unequal number of examples across the different clusters, (b) a fragmented feature space each for clusters 1 and 3, (c) a completely noisy feature, and (d) an overlap between second and third clusters. As shown in Fig. \ref{subspace1d}, CRAFT again identified the subspaces accurately. 

Fig. \ref{subspace2a} shows the second dataset comprising 300 36-feature points, evenly split across 3 clusters, drawn from independent Gaussians having unit variance and means 1, 5 and 10 respectively. We designed clusters to comprise features 1-12, 13-24, and 22-34 respectively so that the first two clusters had disjoint, whereas the last two some overlapping features.  We added isotropic noise by sampling the remaining features from a Gaussian distribution having mean 0 and standard deviation 3.  Fig. \ref{subspace2b} shows that CRAFT recovered the subspaces with $m = 0.33$. We then modified this dataset in Fig. \ref{subspace2c} to have cluster 2 span a non-contiguous feature subspace. Additionally, cluster 2 is designed such that one partition of its features overlaps partially with cluster 1, while the other is subsumed completely within the subspace of cluster 3. Besides, there are several extraneous features not contained within any cluster. CRAFT recovers the subspaces on this data too (Fig. \ref{subspace2d}).   

\noindent \textbf{Approximate Budget Setting:}
We now show that CRAFT may recover the subspaces even when we allow a different number of features to be selected across the different clusters. 

We modified the original categorical synthetic dataset to have cluster 3 (a)  overlap with cluster 1,  and more importantly, (b) significantly overlap with cluster 2.  We obtained the configuration, shown in  Fig. \ref{subspace3a}, by splitting cluster 3 (8 features) evenly in two parts, and increasing the number of features in cluster 2 (16 features) considerably relative to cluster 1 (9 features), thereby making the distribution of features across the clusters non-uniform.  We observed, see Fig. \ref{subspace3b}, that for $\epsilon_c \in [0.76, 1)$, the CRAFT algorithm for the approximate budget setting recovered the subspace exactly for a wide range of $m$, more specifically for all values, when $m$ was varied in increments of 0.1 from $0.2$ to  $0.9$.  This implies the procedure essentially requires tuning only $\epsilon_c$. We easily found the appropriate range by searching in decrements of $0.01$ starting from 1.  Fig. \ref{subspace3d} shows the recovered subspaces for a similar set-up for the numeric data shown in Fig. \ref{subspace3c}. We observed that for $\epsilon_v \in [4, 6]$, the recovery  was robust to selection of $m \in [0.2, 0.9]$, similar to the case of categorical data.   For our purposes, we searched for $\epsilon_v$ in increments of 0.5 from 1 to 9, since the global variance was set to 9. Thus, with minimal tuning, we recovered subspaces in all cases.

\begin{figure*}[t!]
%\centering
\subfigure[Dataset 1]{
   \includegraphics[trim = 0.6in 2.5in 0.1in 2.5in, clip, scale=0.16]{ExactCatOrig2.pdf}
  \label{subspace1c}
 }
 \subfigure[$m$ = 0.3]{
   \includegraphics[trim = 0.6in 2.5in 0.1in 2.5in, clip, scale=0.16]{ExactCat2.pdf}
  \label{subspace1d}  
 }
\subfigure[]{
   \includegraphics[trim = 0.3in 2.5in 0.1in 2.5in, clip, scale=0.16]{ExactCatOrig5.pdf}
   \label{subspace1a}
 }
\subfigure[]{
   \includegraphics[trim = 0.3in 2.5in 0.1in 2.5in, clip, scale=0.16]{ExactCat3.pdf}
   \label{subspace1b}
 }
 \label{}
\caption{\textbf{(Fixed budget)} CRAFT recovered the subspaces on categorical datasets.}
\end{figure*}

\begin{figure*}[t!]
\centering
\subfigure[]{
   \includegraphics[trim = 0.9in 2.5in 0.1in 2.8in, clip, scale=0.16]{ExactNumOrig.pdf}
  \label{subspace2a}
 }
 \subfigure[]{
   \includegraphics[trim = 0.9in 2.5in 0.1in 2.8in, clip, scale=0.16]{ExactNum.pdf}
  \label{subspace2b} 
 }
\subfigure[]{
   \includegraphics[trim = 0.9in 2.5in 0.1in 2.8in, clip, scale=0.16]{ExactNumOrig3.pdf}
   \label{subspace2c}
 }
  \subfigure[]{
   \includegraphics[trim = 0.9in 2.5in 0.1in 2.8in, clip, scale=0.16]{ExactNum3.pdf}
   \label{subspace2d}
 }
 \label{}
\caption{\textbf{(Fixed budget)} CRAFT recovered the subspaces on numeric datasets.}
\end{figure*}


\begin{figure*}[t!]
\centering
\subfigure[]{
   \includegraphics[trim = 0.6in 2.5in 0.1in 2.5in, clip, scale=0.16]{ApproxCatOrig.pdf}
  \label{subspace3a}
 }
 \subfigure[]{
   \includegraphics[trim = 0.6in 2.5in 0.1in 2.5in, clip, scale=0.16]{ApproxCat1.pdf}
  \label{subspace3b} 
 }
\subfigure[]{
   \includegraphics[trim = 0.3in 2.5in 0.1in 2.5in, clip, scale=0.16]{ApproxNumOrig.pdf}
   \label{subspace3c}
 }
  \subfigure[]{
   \includegraphics[trim = 0.3in 2.5in 0.1in 2.5in, clip, scale=0.16]{ApproxNum.pdf}
   \label{subspace3d}
 }
 \label{subspace3}
\caption{\textbf{(Approximate budget)} CRAFT recovered the subspaces on both the categorical dataset shown in (a) and the numeric dataset shown in (c), and required minimal tuning.}    
\end{figure*}

%trim = {0.3in 2.5in 0.1in 0in}, clip, scale=0.21

\begin{figure*}[t]
\centering
\subfigure[$m$ = 0.2]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GPurity02.pdf}
  \label{Comparison1a}
 }
\subfigure[$m$ = 0.4]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GPurity04.pdf}
   \label{Comparison1b}
   }
  \subfigure[$m$ = 0.6]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GPurity06.pdf}
  \label{Comparison1c}
 }
 \subfigure[$m$ = 0.2]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GNMI02.pdf}
  \label{Comparison2a}
 }
\subfigure[$m$ = 0.4]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GNMI04.pdf}
   \label{Comparison2b}
 }
 \subfigure[$m$ = 0.6]{
   \includegraphics[trim = {0.3in 2.5in 0.1in 2.8in}, clip, scale=0.21]{GNMI06.pdf}
  \label{Comparison2c}
 }
\caption{Purity (a-c) and NMI (d-f) comparisons on Splice for different values of $m$. DP-RF is DP-means(R) extended to incorporate feature selection.  \label{Comparison1}}
\end{figure*}

\subsubsection*{Experimental Setup for Real Datasets}
In order to compare the non-parametric CRAFT algorithm with other methods (where the number of clusters K is not defined in advance), we followed the farthest-first heuristic used by the authors of DP-means \cite{Kulis}, which is reminiscent of the seeding proposed in methods such as K-means$++$ \cite{KMeans++} and Hochbaum-Shmoys initialization \cite{HS}: for an approximate number of desired clusters $k$,  a suitable $\lambda$ is found in the following manner. First a singleton set $T$ is initialized, and then iteratively at each of the $k$ rounds, the point in the dataset that is farthest from $T$ is added to $T$. The distance of a point $x$ from $T$ is taken to be the smallest distance between $x$  and any point in $T$, for evaluating the corresponding objective function. At the end of the $k$ rounds, we set $\lambda$ as the distance of the last point that was included in $T$. Thus, for both DP-means and CRAFT, we determined their respective $\lambda$ by following the farthest first heuristic evaluated on their objectives: K-means objective for DP-means and entropy based objective for CRAFT.  

\par \citet{Kulis} initialized $T$ to the global mean for DP-means algorithm. On the other hand, we chose a point randomly from the input to initialize $T$ for CRAFT.  In our experiments, we found that this strategy can be often more effective than using the global mean since the cluster centers tend to be better separated and less constrained.  However, to highlight that the poor performance of DP-means is not just an artifact of the initial cluster selection strategy but more importantly the failure of its squared Euclidean based objective  to deal with categorical data sets, we also conducted experiments on DP-means with random selection of the initial cluster center from the data points. We call this method DP-means(R) where R indicates randomness in selecting the initial center. 

\subsubsection*{Evaluation Criteria For Real Datasets}
To evaluate the quality of clustering, we use datasets with known true labels. We use two standard metrics, \textit{purity} and \textit{normalized mutual information} (NMI), to measure the clustering performance \cite{ManningRaSc08, StrehlGh02}. To compute purity, each full cluster is assigned to the class label that is most frequent in the cluster. Purity is the proportion of examples that we assigned to the correct label. Normalized mutual information is the mutual information between the cluster labeling and the true labels, divided by the square root of the true label entropy times the clustering assignment entropy. Both purity and NMI lie between 0 and 1 - the closer they are to 1, the better the quality of clustering is. 

Henceforth, we use Algorithm \ref{alg3} for the fixed budget setting in our experiments to ensure a fair comparison with the other methods since they presume a fixed $m$. 

\begin{table*}[t!]
\centering
\caption{CRAFT versus DP-means and state-of-the-art feature selection methods when half of the features were selected (i.e. $m = 0.5$). We abbreviate MCFS to M, NDFS to N, DP-means to D, and DP-means(R) to DR to fit the table within margins. DP-means and  DP-means(R) do not select any features. The number of clusters was chosen to be same as the number of classes in each dataset. \label{Table:SpliceAll}}
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|} \hline
\hline
 \textbf{Dataset} &\multicolumn{5}{|c||}{\textbf{Average Purity}}&\multicolumn{5}{|c|}{\textbf{Average NMI}}\\
\cline{2-11} 
 & \textbf{CRAFT} & \textbf{M} & \textbf{N} & \textbf{DR} & \textbf{D} & \textbf{CRAFT} & \textbf{M} & \textbf{N} & \textbf{DR} & \textbf{D}\\
\hline\hline
Bank   &   0.67  &  0.65 &    0.59 &   0.61&   0.61  &  0.16 &   0.06 &    0.02 &    0.03 &   0.03 \\ \hline
Spam    &        0.72 &   0.64 &    0.64 &   0.61 &    0.61 &  0.20 &    0.05 &   0.05 &   0.00 &      0.00\\ \hline
Wine      &       0.72  &  0.72 &    0.69 &    0.66   &       0.66 &  0.48 &    0.35  &  0.47  &  0.44   &    0.44 \\ \hline
Splice    &       0.75  &  0.62  &  0.63   &  0.61    &   0.52  &     0.20  &   0.04  &  0.05  &  0.05    &   0.01 \\ \hline
Monk     &       0.56  &  0.55 &   0.53  &  0.54   &    0.53 &  0.03 &    0.02  &  0.00  &  0.00   &    0.00 \\ \hline
\end{tabular}
\end{table*}

\begin{table*}[t!]
\centering
\caption{CRAFT versus DP-means and state-of-the-art feature selection methods ($m = 0.8$). \label{Table:SpliceAll2}}
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|} \hline
\hline
 \textbf{Dataset} &\multicolumn{5}{|c||}{\textbf{Average Purity}}&\multicolumn{5}{|c|}{\textbf{Average NMI}}\\
\cline{2-11} 
 & \textbf{CRAFT} & \textbf{M} & \textbf{N} & \textbf{DR} & \textbf{D} & \textbf{CRAFT} & \textbf{M} & \textbf{N} & \textbf{DR} & \textbf{D}\\
\hline\hline
Bank   &   0.64  &  0.61 &    0.61 &   0.61&   0.61  &  0.10 &   0.03 &    0.03 &    0.03 &   0.03 \\ \hline
Spam    &        0.72 &   0.64 &    0.64 &   0.61 &    0.61 &  0.23 &    0.05 &   0.05 &   0.00 &      0.00\\ \hline
Wine      &       0.82  &  0.73 &    0.69 &    0.66   &       0.66 &  0.55 &    0.42  &  0.42  &  0.44   &    0.44 \\ \hline
Splice    &       0.74  &  0.68  &  0.63   &  0.61    &   0.52  &     0.18  &   0.09  &  0.05  &  0.05    &   0.01 \\ \hline
Monk     &       0.57  &  0.54 &   0.54  &  0.54   &    0.53 &  0.03 &    0.00  &  0.00  &  0.00   &    0.00 \\ \hline
\end{tabular}
\end{table*}

     
\subsubsection*{Comparison of CRAFT with DP-means extended to Feature Selection} 
 We now provide evidence  that CRAFT outperforms DP-means on categorical data.   We describe in detail the Splice junction determination dataset \cite{Datasets} that has all features categorical. We borrowed the feature selection term from CRAFT to extend DP-means(R) to include feature selection, and retained its squared Euclidean distance measure. Recall that the CRAFT objective degenerates to DP-means(R) on numeric data when all features are retained. Thus, this extended objective is just the CRAFT objective without the categorical term.  Fig. \ref{Comparison1}  shows the comparison results on Splice data for different values of $m$. CRAFT outperforms extended DP-means(R) in terms of both purity and NMI, thereby making the benefits of our entropy based formalism for categorical data conspicuous.  %In particular, our results endorse the applicability of CRAFT for in a nonparametric setting.  


%We first report clustering results on Splice in the absence of feature selection, when the number $k$ of desired clusters is varied between 2 and 10.  Table \ref{Table:DPSplice}  shows the mean and standard deviation values for the different algorithms, where the results are averaged over 20 independent runs  of each algorithm.  Note that since DP-means uses mean of the dataset as the first cluster center, its performance is deterministic for a fixed $\lambda$. 
%The results clearly demonstrate that CRAFT outperforms DP-means and DP-means(R) on both purity and NMI measures.  It is evident that the squared Euclidean distance based objective does not work well for DP-means when dealing with categorical datasets like Splice. 

\subsubsection*{Comparison with State-of-the-Art Unsupervised Feature Selection Methods}
We now demonstrate the benefits of cluster specific  feature selection accomplished by CRAFT.   Table \ref{Table:SpliceAll} and Table \ref{Table:SpliceAll2} show how CRAFT compares with two state-of-the-art unsupervised feature selection methods -  MCFS \cite{MCFS} and NDFS \cite{NDFS} - besides DP-means and DP-means(R) on several datasets \cite{Datasets}, namely Bank, Spam, Wine,  Splice (described above),  and Monk, when $m$ was set to 0.5 and 0.8 respectively.  Clearly, CRAFT outperformed all the methods with respect to both Purity and NMI. Our experiments clearly highlight that CRAFT (a) works well for both numeric and categorical data, and (b) outperforms both the global feature selection algorithms and clustering methods, such as DP-means, that do not select features. 

Finally, in our experiments, we found that besides performance,  CRAFT also compared favorably with both the feature selection methods, MCFS and NDFS, in terms of time requirements. For instance, on the Spam dataset for $m=0.5$, CRAFT required an average execution time of only 0.49 seconds, compared to 2.16 and 61.41 seconds by MCFS and NDFS respectively.  This behavior can be attributed primarily to the benefits of the scalable K-means style algorithm employed by CRAFT, as opposed to MCFS and NDFS that require computation-intensive spectral algorithms.   

 % %We observe that the methods that select features, i.e. CRAFT, MCFS and NDFS, typically did much better than DP-means and DP-means (R), the two methods that cluster data points using all the features. Among the unsupervised feature selection methods, CRAFT performed the best.

 %  Splice   is a computational biology dataset, and  features are categorical. The attributes encode DNA sequences, and the label encodes whether the sequence is an EI boundary or IE boundary. All the features are categorical because they encode a DNA sequence. We treated feature values 1 and 2 with 0, and 3 and 4 with 1 to create a binary dataset. 

%\footnote{https://archive.ics.uci.edu/ml/datasets/banknote+authentication}
%\footnote{https://archive.ics.uci.edu/ml/datasets/Spambase}
%\footnote{https://archive.ics.uci.edu/ml/datasets/Wine} 
%\footnote{https://archive.ics.uci.edu/ml/datasets/Congressional+Voting+Records}
%\footnote{https://archive.ics.uci.edu/ml/datasets/Soybean+(Small)} 
%\footnote{https://archive.ics.uci.edu/ml/datasets/MONK's+Problems}






%We conducted two sets of experiments, one where the number of clusters is chosen manually, and the other where it is chosen non-parametrically. We start with the case where the number of clusters is chosen manually, both for CAKE (without feature selection) and K-means. 
%
%
%
%
%
% In Table  \ref{Table:FixedKSplice} Analogous results for splice are presented in Table. 
%
%Across every choice of K, CAKE's performance dominated that of K-means, unsurprisingly since the features are categorical. K-modes did not perform well, even though it was designed for categorical data. For instance, Fig. \ref{fig:kmodes} demonstrates K-modes performs poorly on splice in terms of purity.  Since we did not find K-modes to be competitive, we omit any further discussion on K-modes in the sequel.
%
%We note that we did find datasets where the choice of algorithm did not show improvement. Namely, when the datasets were small, all of the algorithms performed similarly, and there was no significant difference in performance. It seems that performance differences between algorithms are revealed mainly for larger datasets.


%
%\begin{table*}
%\centering
%%\ra{1.3}
%\caption{CAKE vs.~K-means on Adult Dataset\label{Table:FixedKAdult}}
%\begin{tabular}{|c|c|c||c|c|} \hline
%\hline
% \textbf{Clusters} &\multicolumn{2}{|c||}{\textbf{Purity}}&\multicolumn{2}{|c|}{\textbf{NMI}}\\
%\cline{2-5}
% &\textbf{CAKE} &\textbf{K-means} & \textbf{CAKE} &\textbf{K-means}\\
%\hline\hline
%3       &     0.7571 +/- 0.016   &   0.7525 +/- 0.002  &      0.111 +/- 0.025  &  0.095 +/- 0.024 \\ \hline
%  4      &    0.7679 +/- 0.020    & 0.7547 +/- 0.004  &   0.105 +/- 0.019   & 0.095 +/- 0.006  \\ \hline   
%  5      &       0.7660 +/- 0.020  &   0.7572 +/- 0.006   &  0.101 +/- 0.012  &  0.091 +/- 0.009   \\ \hline 
%  6      &       0.7756 +/- 0.024   &  0.7612 +/- 0.011   & 0.100 +/- 0.011   & 0.087 +/- 0.007    \\ \hline
%  7     &     0.7770 +/- 0.023  &   0.7599 +/- 0.009    &  0.096 +/- 0.014   & 0.086 +/- 0.008    \\ \hline 
%  8      &      0.7741 +/- 0.019 &    0.7616 +/- 0.009   & 0.094 +/- 0.009   & 0.085 +/- 0.007     \\ \hline
%  9      &      0.7771 +/- 0.019  &   0.7616 +/- 0.007    & 0.093 +/- 0.009   & 0.084 +/- 0.007    \\ \hline
%  10     &      0.7801 +/- 0.01   &   0.7641 +/- 0.009    &  0.093 +/- 0.011  &  0.084 +/- 0.007    \\ \hline
%  \end{tabular}
%\end{table*}
 
%\begin{table*}
%\centering
%\caption{CAKE vs.~K-means on Splice  Dataset\label{Table:FixedKSplice}}
%\begin{tabular}{|c|c|c||c|c|} \hline
%\hline
% \textbf{Clusters} &\multicolumn{2}{|c||}{\textbf{Purity}}&\multicolumn{2}{|c|}{\textbf{NMI}}\\
%\cline{2-5}
% &\textbf{CAKE} &\textbf{K-means} & \textbf{CAKE} &\textbf{K-means}\\
%\hline\hline
%3       &     0.7666 +/- 0.063    &   0.7203 +/- 0.044  &     0.217 +/- 0.103    &   0.156 +/- 0.083 \\ \hline
%  4      &    0.7555 +/- 0.045    & 0.7252 +/- 0.018  &    0.193 +/- 0.066   & 0.174 +/- 0.041  \\ \hline   
%  5      &      0.7618 +/- 0.043   &  0.7454 +/- 0.030   &  0.180 +/- 0.046   &  0.163 +/- 0.031   \\ \hline 
%  6      &      0.7606 +/- 0.037   &  0.7431 +/- 0.028   & 0.167 +/- 0.033   &  0.148 +/- 0.026    \\ \hline
%  7     &     0.7770 +/- 0.040   &  0.7429 +/- 0.026    &  0.169 +/- 0.037   &  0.137 +/- 0.025    \\ \hline 
%  8      &      0.7677 +/- 0.042  &   0.7355 +/- 0.030    & 0.152 +/- 0.035 &    0.122 +/- 0.020     \\ \hline
%  9      &      0.7649 +/- 0.037   &  0.7421 +/- 0.021    & 0.145 +/- 0.031   &  0.123 +/- 0.017    \\ \hline
%  10     &      0.7717 +/- 0.031   &  0.7474 +/- 0.022    &  0.140 +/- 0.020   &  0.121 +/- 0.015    \\ \hline
%  \end{tabular}
%\end{table*}
 





%\begin{table*}
%\centering
%\caption{DP-CAKE vs.~DP-means and DP-means(R) on Adult Dataset. Note that DP-means is deterministic, unlike DP-CAKE, since global mean is used as the first cluster center, and the data set points are subsequently processed in the fixed input order. Hence there is no standard deviation for DP-means. DP-means(R) is DP-means with a random initialization: we choose a point randomly from the dataset as the first center, and therefore we achieve random orderings in which points are processed and (possibly) different clusterings. Also, depending on the data, the different clusterings may still have the same purity (as seen here for DP-means(R)) and/or NMI. \label{Table:DPAdult}}
%\begin{tabular}{|c|c|c|c||c|c|c|} \hline
%\hline
% \textbf{Clusters} &\multicolumn{3}{|c||}{\textbf{Purity}}&\multicolumn{3}{|c|}{\textbf{NMI}}\\
%\cline{2-7}
% &\textbf{DP-CAKE} &\textbf{DP-means} & \textbf{DP-means(R)} & \textbf{DP-CAKE} &\textbf{DP-means} & \textbf{DP-means(R)}\\
%\hline\hline
%3       &        0.7523 +/- 0.001 &    0.7520  &  0.7520 +/- 0.000 & 0.111 +/- 0.013  &      0.094  &   0.020 +/- 0.048 \\ \hline
%  4       &      0.7520 +/- 0.000  &   0.7604  & 0.7520 +/- 0.000 & 0.108 +/- 0.012    &     0.080   & 0.026 +/- 0.054 \\ \hline
%  5       &      0.7534 +/- 0.003   &  0.7605   & 0.7520 +/- 0.000 & 0.108 +/- 0.011    &    0.082  &  0.048 +/- 0.064 \\ \hline
%  6       &       0.7648 +/- 0.023  &  0.7604  & 0.7520 +/- 0.000 & 0.106 +/- 0.008    &     0.088    &  0.048 +/- 0.064 \\ \hline
%  7       &       0.7617 +/- 0.020  &   0.7520  & 0.7520 +/- 0.000 &  0.105 +/- 0.009    &   0.097   &  0.048 +/- 0.064 \\ \hline
%  8       &       0.7683 +/- 0.022   &  0.7520  & 0.7520 +/- 0.000 & 0.104 +/- 0.008    &    0.100   &  0.050 +/- 0.063 \\ \hline
%  9       &       0.7669 +/- 0.020   & 0.7611   & 0.7520 +/- 0.000 & 0.102 +/- 0.010     &   0.089   & 0.053 +/- 0.062 \\ \hline
%  10     &       0.7730 +/- 0.023   &  0.7520  & 0.7520 +/- 0.000 & 0.099 +/- 0.010     &   0.091  &  0.053 +/- 0.062 \\ \hline
%  \end{tabular}
%\end{table*}
%





%\subsubsection*{Feature Selection}
%Next we describe the performance of FDP-CAKE. Since we are especially interested in demonstrating the impact of local feature selection on the quality of clustering, we present the results for $\rho$ set close to $m(1-m)$, thus allowing for maximum permissible variance in features across the clusters.  Table \ref{Table:FDP} documents the results of our experiments with the two datasets for $m = 0.9$ ($\sim 10\%$ reduction in the number of features on average). Fig.~\ref{fig:FDP} displays the performance of all non-parametric algorithms in perspective - we see that DP-CAKE and FDP-CAKE outperform DP-means and DP-means(R) in terms of both purity and NMI. Interestingly, while FDP-CAKE with $20\%$ average feature reduction ($m = 0.8$) performs as well as  FDP-CAKE with $10\%$ reduction ($m$ = 0.9) and DP-CAKE when evaluated for purity, it improves over their NMI for most values of K. This substantiates our assertion that local feature selection helps improve the quality of clustering, and underlines the efficacy of the CAKE framework. 
%\begin{figure*}[t!]
%   % \centering
%    \begin{subfigure}[t]{0.5\textwidth}
%        \centering
%        \includegraphics[trim = 0.1in 2.5in 0.1in 2.5in, clip, scale=0.5]{Plot_Purity_All_Splice.pdf}
%        \caption{Purity}
%    \end{subfigure}%
%    ~ 
%    \begin{subfigure}[t]{0.5\textwidth}
%        \centering
%        \includegraphics[trim = 0.1in 2.5in 0.1in 2.5in, clip, scale=0.5]{Plot_NMI_All_Splice.pdf}
%        \caption{NMI}
%    \end{subfigure}
%    \caption{Comparison of the algorithms on Splice in terms of: (a) Purity and (b) NMI. The two FDP-CAKE curves, corresponding to $m = 0.8$ and $m = 0.9$ were generated by setting $\rho=\min \left[\dfrac{m(1-m)^2}{2-m}, \dfrac{m^2(1-m)}{1+m}\right]$ to allow for maximum variance toward achieving cluster specific feature selection. Clearly, despite considerable average feature reduction (20\% when $m = 0.8$, and 10\% when $m=0.9$), FDP-CAKE outperforms its DP-means counterparts on both NMI and purity.}
%    \label{fig:FDP}
%\end{figure*}

%\begin{figure*}[t!]
%%\centering
%\subfigure[Purity]{
%   \includegraphics[trim = 0.3in 2.5in 0.1in 2.5in, clip, scale=0.43]{Plot_Purity_All_Splice.pdf}
%   \label{fig:FDP_purity}
% }
%~
% \subfigure[NMI]{
%   \includegraphics[trim = 0.6in 2.5in 0.1in 2.5in, clip, scale=0.45]{Plot_NMI_All_Splice.pdf}
%   \label{fig:FDP_NMI}
% }
%
%\label{fig:FDP}
%\caption{Comparison of the algorithms on Splice in terms of: (a) Purity and (b) NMI. The two FDP-CAKE curves, corresponding to $m = 0.8$ and $m = 0.9$ were generated by setting $\rho$ close to $m(1-m)$ to allow for maximum variance toward achieving cluster specific feature selection. Clearly, despite considerable average feature reduction (20\% when $m = 0.8$, and 10\% when $m=0.9$), FDP-CAKE outperforms its DP-means counterparts on both NMI and purity.}
%\end{figure*}





%\begin{table*}
%\centering
%%\ra{1.3}
%\caption{Performance of FDP-CAKE $(m = 0.9)$ \label{Table:FDP}}
%\begin{tabular}{|c|c|c||c|c|} \hline
%\hline
% \textbf{Clusters} &\multicolumn{2}{|c||}{\textbf{Splice Junction}}&\multicolumn{2}{|c|}{\textbf{Adult}}\\
%\cline{2-5}
% &\textbf{Purity} &\textbf{NMI} & \textbf{Purity} &\textbf{NMI}\\
%\hline\hline
%3 &  0.7532 +/- 0.053 & 0.177 +/- 0.063 & 0.7564 +/- 0.014 & 0.104 +/- 0.022  \\ \hline
% 4 &  0.7803 +/- 0.053 & 0.197 +/- 0.062 & 0.7539 +/- 0.004 & 0.102 +/- 0.019 \\ \hline
% 5 &  0.7815 +/- 0.036 & 0.181 +/- 0.047 & 0.7583 +/- 0.013 & 0.106 +/- 0.011 \\ \hline
% 6 &  0.7756 +/- 0.031 & 0.172 +/- 0.039 & 0.7674 +/- 0.018 & 0.100 +/- 0.012 \\ \hline
% 7 &  0.7664 +/- 0.034 & 0.153 +/- 0.036 & 0.7659 +/- 0.017 & 0.101 +/- 0.011 \\ \hline
% 8 &  0.7718 +/- 0.020 & 0.150 +/- 0.024 & 0.7647 +/- 0.016 & 0.100 +/- 0.011 \\ \hline
% 9 &  0.7619 +/- 0.027 & 0.137 +/- 0.033 & 0.7652 +/- 0.017 & 0.099 +/- 0.011 \\ \hline
% 10&  0.7682 +/- 0.032 & 0.143 +/- 0.032 & 0.7662 +/- 0.016 & 0.095 +/- 0.009 \\ \hline
%  \end{tabular}
%\end{table*}

%\newpage
 %\clearpage 

% The following two commands are all you need in the
% initial runs of your .tex file to
% produce the bibliography for the citations in your paper.
%\newpage
  % sigproc.bib is the name of the Bibliography in this case
% You must have a proper ".bib" file
%  and remember to run:
% latex bibtex latex latex
% to resolve all references
%



==> introduction_V.tex <==
\section{Introduction}
%Feature selection, known variously as variable selection, attribute selection, or variable subset selection, remains a central theme for most machine learning tasks, especially those dealing with high dimensional data. Besides ensuring storage savings, and therefore reduced data processing and communication overheads, feature selection provides several other benefits such as improving prediction performance by ameliorating the curse of dimensionality, and enhancing data interpretability by facilitating data visualization. Indeed, feature selection has garnered great interest from the learning community, as evident from some highly cited surveys  \cite{Guyon, Liu}.  
%
    
Our primary goal is to present a principled framework for unsupervised feature selection. Feature selection can be global (same features across clusters) or local (cluster-specific features).  For most real world applications, feature selection should be cluster specific, e.g., when clustering news articles, the similarity between articles about politics should be assessed based on the language about politics, regardless of their references to other topics such as sports. Unsupervised global feature selection is widely considered a hard problem \cite{NDFS}. Cluster-specific unsupervised feature selection is even harder since separate, possibly overlapping, subspaces need to be inferred. Using an adjustable parameter, our proposed framework CRAFT can achieve either global or local feature selection. %Essentially, CRAFT performs a type of subspace clustering when choosing local features. 

Simultaneously, CRAFT addresses another long standing challenge for clustering methodology: how to handle assorted data, i.e., data containing both numeric and categorical features. The machine learning literature abounds in algorithms on clustering, however, a vast majority of these methods are designed exclusively for numeric data.  This is often problematic since most real world datasets contain categorical variables or are processed to contain categorical variables; for instance, in web-based clustering applications, the representation of each document (webpage) as a binary (categorical) feature vector is completely standard. Treating categorical data as if it were real-valued simply does not work due to absence of any ordinal relationships among the categorical labels. This explains, in part, why despite several attempts  \cite{Ahmad,Aranganayagi,Huang1,Huang2,San}, the popular clustering methods such as the K-means \cite{Lloyd,Macqueen} have largely proved ineffective in handling categorical data. %leading to specifically designed distance metrics for such data \cite{Boriah}. 

The derivation of our algorithms follows from asymptotics on the log posterior of our generative model. The model is based on Dirichlet process mixtures \cite{Guan, Shaf, Sohn} (see \citet{Kim14} for a prototype-based generative model), and thus the number of clusters can be chosen non-parametrically by the algorithm. Our asymptotic calculations significantly extend the works of \citet{Kulis}, who derived the DP-means objective by considering approximations to the log-likelihood, and \citet{Broderick}, who instead approximated the posterior log likelihood to derive other nonparametric variations of K-means. Our derivation differs from both these works since they are not designed for feature selection, and our generative model is entirely different as well.  When the data are completely numeric, we recover the DP-means objective with an additional term arising due to feature selection.   In general, the asymptotics yield interpretable objective functions, and suggest K-means style algorithms that outperform several state-of-the-art benchmarks. %The resulting algorithm scales nicely and is simple to implement like K-means.  In particular, our algorithm with cluster-specific feature selection has the following main steps repeated until convergence: compute the ``distances"  to the cluster centers using the selected features for each cluster, choose which cluster each point should be assigned (and create new clusters if needed), and recompute the cluster centers and select the appropriate cluster-specific features for the next iteration. 


%\subsection{Contributions and Organization}
%We make the following main contributions in this paper.
%\begin{itemize}
%\item We derive principled K-means-like algorithms to handling mix (i.e. both categorical and numeric) data.
%\item We show how feature selection can be performed as a part of the algorithm. There are adjustable parameters that govern whether feature selection is mostly local to the cluster, or global over all clusters.
%\item We combine these ideas with the work on Dirichlet process priors so that the number of clusters does not need to be predetermined.
%\item We present experiments indicating that our approaches are very promising, and outperform the K-means algorithm and its nonparametric analogue.
%\end{itemize}


% ---------- The following text was removed from NIPS submission

%We first motivate our framework, CRAFT, specifically in the context of clustering binary categorical data without feature selection, and outline a simple K-means style algorithm in Section \ref{SectionBasicCRAFT}.  We then proceed to the more general version that accomplishes joint clustering and feature selection in Section \ref{SectionCRAFTWithFS},  and present a feature selection algorithm that handles both numeric and categorical data.  We provide a detailed experimental analysis in Section \ref{SectionExperiments}. All the derivations are given in the Supplementary Section \ref{Supplementary}.  

% -----------



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]


% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


